Paraphrasing vs Coreferring: Two Sides of the Same Coin

We study the potential synergy between two different NLP tasks, both confronting predicate lexical variability: identifying predicate paraphrases, and event coreference resolution. First, we used annotations from an event coreference dataset as distant supervision to re-score heuristically-extracted predicate paraphrases. The new scoring gained more than 18 points in average precision upon their ranking by the original scoring method. Then, we used the same re-ranking features as additional inputs to a state-of-the-art event coreference resolution model, which yielded modest but consistent improvements to the model's performance. The results suggest a promising direction to leverage data and models for each of the tasks to the benefit of the other.

==> a-appendices.tex <==
The full feature list of a given predicate paraphrase pair $p_1, p_2$ (Section~\ref{sec:features}) includes features from several categories:

\subsection{Features from Chirps}
\label{sec:appendix_chirps_features}

\begin{enumerate}
    \item \textbf{Number of templates}: the number of different predicate paraphrase pairs with $p_1$ and $p_2$ as predicates, regardless of argument ordering, e.g. \{ [a$_0$] release [a$_1$] / [a$_0$] reveal [a$_1$], release [a$_0$] [a$_1$] / reveal [a$_0$] [a$_1$] \} yield 2. 
    \item \textbf{Number of supporting pairs}: the total number of support pairs of $p_1$ and $p_2$ across the template variants.
    \item \textbf{Number of days}: the total number of days $d$ that $p_1$ and $p_2$ was matched in Chirps across the template variants.
    \item \textbf{Score}: the maximal Chirps score across the template variants. 
    \item \textbf{Number of available supporting pairs}: the number of support pairs of $p_1$ and $p_2$ across the template variants \emph{that were still available to download}. 
    \item \textbf{Days of available supporting pairs}: the total number of days $d$ in which the support pairs above occurred in the available tweets. 
\end{enumerate}

\subsection{Named Entity Features} 
\label{sec:appendix_ne_features}

As described in Section~\ref{sec:features}:

\begin{enumerate}
\setcounter{enumi}{6}
    \item \textbf{Above Threshold}: number of pairs with NEC  score of at least $T$.
    \item \textbf{Average Above Threshold}: average of NEC scores for pairs with a score of at least $T$. 
    \item \textbf{Perfectly Clustered with NE Coverage}: the number of pairs with NEC score of at least $T$ \textbf{and} perfect clustering for event coreference resolution (Section~\ref{sec:appendix_coref_features}).
\end{enumerate}

\subsection{Graph Features} 
\label{sec:appendix_graph_features}

As described in Section~\ref{sec:features}:

\begin{enumerate}
\setcounter{enumi}{9}
    \item \textbf{Number of connected components}: ${\operatorname{\#connected}(p_1, p_2)= |\{c \in C : |c| > 2\}|}$
    \item \textbf{Average connected component}: the average size of connected components in $G_{p_1, p_2}$.
    \item \textbf{In Clique}: the number of pairs in $\operatorname{support-pairs}(p_1, p_2)$ that are in a clique. 
\end{enumerate}

\subsection{Cross-document Coreference Features}
\label{sec:appendix_coref_features}

As described in Section~\ref{sec:features}:

\begin{enumerate}
\setcounter{enumi}{12}
    \item \textbf{Event Perfect}: number of event pairs with perfect match. 
    \item \textbf{Event No Match}: number of event pairs with no match.
    \item \textbf{Entity Perfect}: number of entity pairs with perfect match. 
    \item \textbf{Entity Reverse}: number of entity pairs with reverse match. 
    \item \textbf{Entity No Match}: number of entity pairs with no match.
\end{enumerate}





==> figures/chirps_coverage.tex <==
\setlength\tabcolsep{2pt}
\begin{tabular}{@{}l|lll|lll|lll@{}}
\toprule
& \multicolumn{3}{c}{\textbf{Train}} & \multicolumn{3}{c}{\textbf{Dev}} & \multicolumn{3}{c}{\textbf{Test}} \\ 
& Covered & Total & \% & Covered & Total & \% & Covered & Total & \%   \\ \midrule
verbal & 371  & 715 & 51.9 & 124 & 231 & 53.7 & 196 & 354 & 55.4 \\
all & 385 & 1195 & 32.2 & 132  & 390 & 33.8 & 199  & 702 & 28.3 \\ \bottomrule
\end{tabular}

==> figures/errors.tex <==
\setlength\tabcolsep{6pt}
\begin{table*}[t]
\centering
\small
\begin{tabular}{lc}
\toprule
\multicolumn{2}{c}{\textbf{False Positive Examples}} \\ 
\midrule
S$_1$: [...] a jury's decision to execute Scott Peterson for the \underline{murder} of his pregnant wife. & \multirow{2}{*}{0.237} \\
S$_2$: found guilty of first-degree murder, [...] he deserves to \underline{die} for his crimes. & \\
\midrule
S$_1$: [...] Polygamist leader Warren Jeffs \underline{sentenced} to life in prison. & \multirow{2}{*}{0.882} \\
S$_2$: Warren Jeffs, [...], \underline{convicted} of sexually assaulting two girls [...]. & \\
\midrule
S$_1$: [...] days after a powerful quake \underline{leveled} buildings and killed one person [...]. & \multirow{2}{*}{0.112} \\
S$_2$: A series of powerful earthquakes [...] injuring dozens and \underline{destroying} hundreds of buildings. & \\
\midrule
\multicolumn{2}{c}{\textbf{False Negative Examples}} \\ 
\midrule
S$_1$: Indonesia's West Papua province was \underline{hit} by a magnitude 6.1 earthquake today. & \multirow{2}{*}{0.272} \\
S$_2$:  the latest powerful tremor to \underline{shake} the region where five people were killed [...]. & \\
\midrule
S$_1$: Apple Inc. [...] \underline{unveiled} a 17-inch MacBook Pro on Tuesday. & \multirow{2}{*}{0.575} \\
S$_2$: The firm \underline{announced} a widely expected refresh of its 17in MacBook Pro [...]. & \\
\midrule
S$_1$: T - Mobile BlackBerry Q10 Pre - Order \underline{Begins} April 29th for Business Customers. & \multirow{2}{*}{0.469} \\
S$_2$: T - Mobile has announced [...] Q10, with pre-registration \underline{starting} on April 29th. & \\
\bottomrule
\end{tabular}
\caption{Examples of false positive and false negative errors on ECB+ recovered by Chirps, together with the cosine similarity scores between the predicates, using GloVe \cite{pennington-etal-2014-glove}.}
\label{tab:errors}
\end{table*}
